The Surprising Effectiveness of Equivariant Models in Domains with Latent Symmetry

Extensive work has demonstrated that equivariant neural networks can significantly improve sample efficiency and generalization by enforcing an inductive bias in the network architecture. These applications typically assume that the domain symmetry is fully described by explicit transformations of the model inputs and outputs. However, many real-life applications contain only latent or partial symmetries which cannot be easily described by simple transformations of the input. In these cases, it is necessary to learn symmetry in the environment instead of imposing it mathematically on the network architecture. We discover, surprisingly, that imposing equivariance constraints that do not exactly match the domain symmetry is very helpful in learning the true symmetry in the environment. We differentiate between extrinsic and incorrect symmetry constraints and show that while imposing incorrect symmetry can impede the model's performance, imposing extrinsic symmetry can actually improve performance. We demonstrate that an equivariant model can significantly outperform non-equivariant methods on domains with latent symmetries both in supervised learning and in reinforcement learning for robotic manipulation and control problems.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> note.tex <==
ground truth function, input distribution, some model, Wasserstein distance

Correct Equi
Incorrect Equi
Extrinsic Equi

Symmetry Corruption


Object Transformation
image transformation

==> old_tables.tex <==
\begin{table}[t]
\centering
\begin{tabular}{cccccc}
\toprule
\multicolumn{2}{c}{Corruption}                    & no corrupt           & grid                 & occlusion            & light effect         \\\midrule
\multirow{2}{*}{100 Data}  & Equi                 & $0.865 \pm 0.025$    & $0.856 \pm 0.023$    & $0.835 \pm 0.034$    & $0.870 \pm 0.012$    \\
                          & CNN                  & $0.419 \pm 0.017$    & $0.422 \pm 0.017$    & $0.419 \pm 0.018$    & $0.424 \pm 0.022$    \\\midrule
\multirow{2}{*}{200 Data}  & Equi                 & $0.947 \pm 0.008$    & $0.938 \pm 0.005$    & $0.946 \pm 0.014$    & $0.920 \pm 0.011$    \\
                          & CNN                  & $0.584 \pm 0.040$    & $0.561 \pm 0.032$    & $0.529 \pm 0.037$    & $0.577 \pm 0.038$    \\\midrule
\multirow{2}{*}{500 Data}  & Equi                 & $0.994 \pm 0.004$    & $0.990 \pm 0.005$    & $0.984 \pm 0.006$    & $0.991 \pm 0.002$    \\
                          & CNN                  & $0.760 \pm 0.041$    & $0.760 \pm 0.051$    & $0.771 \pm 0.058$    & $0.745 \pm 0.051$    \\\midrule
\multirow{2}{*}{1000 Data} & Equi                 & $0.989 \pm 0.005$    & $0.990 \pm 0.003$    & $0.987 \pm 0.011$    & $0.991 \pm 0.004$    \\
                          & CNN                  & $0.861 \pm 0.015$    & $0.860 \pm 0.030$    & $0.841 \pm 0.030$    & $0.880 \pm 0.015$    \\\bottomrule\toprule
\multicolumn{2}{c}{Corruption}                    & squeeze              & reflect              & condition reverse    & side                 \\\midrule
\multirow{2}{*}{100 Data}  & Equi                 & $0.694 \pm 0.015$    & $0.877 \pm 0.017$    & $0.387 \pm 0.034$    & $0.515 \pm 0.021$    \\
                          & CNN                  & $0.421 \pm 0.022$    & $0.425 \pm 0.014$    & $0.221 \pm 0.019$    & $0.441 \pm 0.022$    \\\midrule
\multirow{2}{*}{200 Data}  & Equi                 & $0.865 \pm 0.006$    & $0.937 \pm 0.004$    & $0.447 \pm 0.026$    & $0.694 \pm 0.033$    \\
                          & CNN                  & $0.519 \pm 0.029$    & $0.560 \pm 0.036$    & $0.287 \pm 0.023$    & $0.556 \pm 0.017$    \\\midrule
\multirow{2}{*}{500 Data}  & Equi                 & $0.944 \pm 0.010$    & $0.985 \pm 0.005$    & $0.507 \pm 0.008$    & $0.826 \pm 0.031$    \\
                          & CNN                  & $0.715 \pm 0.050$    & $0.752 \pm 0.031$    & $0.504 \pm 0.036$    & $0.720 \pm 0.029$    \\\midrule
\multirow{2}{*}{1000 Data} & Equi                 & $0.974 \pm 0.007$    & $0.995 \pm 0.002$    & $0.480 \pm 0.017$    & $0.919 \pm 0.011$    \\
                          & CNN                  & $0.844 \pm 0.027$    & $0.864 \pm 0.014$    & $\mathbf{0.619 \pm 0.029}$    & $0.807 \pm 0.031$   \\\bottomrule
\end{tabular}
\caption{Comparison of equivariant network (Equi) and conventional CNN (CNN) trained using different number of training data in the rotation prediction task. Each cell shows the prediction accuracy in the test set Averaged over four seeds.}
\label{tab:sl_equi_vs_cnn}
\end{table}

\begin{table}[t]
\begin{tabular}{clccc}
\toprule
\multicolumn{2}{c}{Corruption}                      & no corrupt        & condition reverse & side              \\\midrule
\multirow{6}{*}{100 Data} & Equi                   & $0.865 \pm 0.025$ & $0.387 \pm 0.034$ & $0.515 \pm 0.021$ \\
                          & CNN                    & $0.419 \pm 0.017$ & $0.221 \pm 0.019$ & $0.441 \pm 0.022$ \\
                          & CNN + img trans        & $0.661 \pm 0.065$ & $0.381 \pm 0.027$ & $0.454 \pm 0.045$ \\\cmidrule{2-5}
                          & Equi + crop            & $\mathbf{0.912 \pm 0.021}$ & $\mathbf{0.405 \pm 0.012}$ & $\mathbf{0.645 \pm 0.024}$ \\
                          & CNN + crop             & $0.512 \pm 0.068$ & $0.316 \pm 0.035$ & $0.491 \pm 0.041$ \\
                          & CNN + crop + img trans & $0.830 \pm 0.028$ & $0.391 \pm 0.018$ & $0.554 \pm 0.031$\\\midrule
\multirow{6}{*}{200 Data}  & Equi                   & $0.947 \pm 0.008$ & $0.447 \pm 0.026$ & $0.694 \pm 0.033$ \\
                          & CNN                    & $0.584 \pm 0.040$ & $0.287 \pm 0.023$ & $0.556 \pm 0.017$ \\
                          & CNN + img trans        & $0.844 \pm 0.044$ & $0.452 \pm 0.014$ & $0.635 \pm 0.046$ \\\cmidrule{2-5}
                          & Equi + crop            & $\mathbf{0.972 \pm 0.015}$ & $\mathbf{0.467 \pm 0.020}$ & $\mathbf{0.801 \pm 0.028}$ \\
                          & CNN + crop             & $0.690 \pm 0.031$ & $0.412 \pm 0.048$ & $0.647 \pm 0.036$ \\
                          & CNN + crop + img trans & $0.954 \pm 0.016$ & $0.454 \pm 0.025$ & $0.737 \pm 0.011$ \\\midrule
\multirow{6}{*}{500 Data}  & Equi                   & $0.994 \pm 0.004$ & $0.507 \pm 0.008$ & $0.826 \pm 0.031$ \\
                          & CNN                    & $0.760 \pm 0.041$ & $0.504 \pm 0.036$ & $0.720 \pm 0.029$ \\
                          & CNN + img trans        & $0.974 \pm 0.006$ & $0.511 \pm 0.013$ & $0.851 \pm 0.023$ \\\cmidrule{2-5}
                          & Equi + crop            & $\mathbf{0.994 \pm 0.003}$ & $0.527 \pm 0.020$ & $0.911 \pm 0.013$ \\
                          & CNN + crop             & $0.861 \pm 0.018$ & $\mathbf{0.672 \pm 0.011}$ & $0.771 \pm 0.019$ \\
                          & CNN + crop + img trans & $0.987 \pm 0.003$ & $0.524 \pm 0.021$ & $\mathbf{0.954 \pm 0.009}$ \\\bottomrule
% \multirow{6}{*}{1000 Data} & Equi                   & $0.989 \pm 0.005$ & $0.480 \pm 0.017$ & $0.919 \pm 0.011$ \\
%                           & CNN                    & $0.861 \pm 0.015$ & $0.619 \pm 0.029$ & $0.807 \pm 0.031$ \\
%                           & CNN + img trans        & $0.990 \pm 0.005$ & $0.487 \pm 0.013$ & $0.926 \pm 0.018$ \\\cmidrule{2-5}
%                           & Equi + crop            & $0.996 \pm 0.002$ & $0.494 \pm 0.015$ & $0.962 \pm 0.008$ \\
%                           & CNN + crop             & $0.937 \pm 0.018$ & $0.814 \pm 0.010$ & $0.914 \pm 0.002$ \\
%                           & CNN + crop + img trans & $0.994 \pm 0.003$ & $0.510 \pm 0.015$ & $0.985 \pm 0.003$\\\bottomrule
\end{tabular}
\caption{Comparison between equivariant network (Equi), conventional CNN (CNN), conventional CNN with image transformation augmentation, and the three methods equipped with random crop augmentation. Each cell shows the prediction accuracy in the test set. Averaged over four seeds.}
\label{tab:sl_aug}
\end{table}

\begin{table}[t]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{cclccccc}
\toprule
\multicolumn{3}{c}{corruption}                                          & no corrupt        & grid              & occlusion          & random light color & light effect      \\\midrule
\multirow{6}{*}{100 data}  & \multirow{3}{*}{no crop} & equi            & $0.865 \pm 0.025$ & $0.856 \pm 0.023$ & $0.835 \pm 0.034$  & $0.832 \pm 0.010$  & $0.870 \pm 0.012$ \\
                           &                          & cnn             & $0.419 \pm 0.017$ & $0.422 \pm 0.017$ & $0.419 \pm 0.018$  & $0.379 \pm 0.026$  & $0.424 \pm 0.022$ \\
                           &                          & cnn + img trans & $0.661 \pm 0.065$ & $0.640 \pm 0.082$ & $0.639 \pm 0.090$  & $0.614 \pm 0.067$  & $0.649 \pm 0.075$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.912 \pm 0.021$ & $0.907 \pm 0.021$ & $0.894 \pm 0.023$  & $0.890 \pm 0.024$  & $0.909 \pm 0.015$ \\
                           &                          & cnn             & $0.512 \pm 0.068$ & $0.507 \pm 0.058$ & $0.510 \pm 0.055$  & $0.464 \pm 0.044$  & $0.510 \pm 0.067$ \\
                           &                          & cnn + img trans & $0.830 \pm 0.028$ & $0.799 \pm 0.016$ & $0.791 \pm 0.039$  & $0.734 \pm 0.032$  & $0.816 \pm 0.030$ \\\midrule
\multirow{6}{*}{200 data}  & \multirow{3}{*}{no crop} & equi            & $0.947 \pm 0.008$ & $0.938 \pm 0.005$ & $0.946 \pm 0.014$  & $0.950 \pm 0.009$  & $0.920 \pm 0.011$ \\
                           &                          & cnn             & $0.584 \pm 0.040$ & $0.561 \pm 0.032$ & $0.529 \pm 0.037$  & $0.499 \pm 0.059$  & $0.577 \pm 0.038$ \\
                           &                          & cnn + img trans & $0.844 \pm 0.044$ & $0.849 \pm 0.014$ & $0.787 \pm 0.045$  & $0.825 \pm 0.031$  & $0.830 \pm 0.038$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.972 \pm 0.015$ & $0.960 \pm 0.013$ & $0.964 \pm 0.006$  & $0.981 \pm 0.007$  & $0.967 \pm 0.012$ \\
                           &                          & cnn             & $0.690 \pm 0.031$ & $0.681 \pm 0.034$ & $0.676 \pm 0.014$  & $0.637 \pm 0.040$  & $0.696 \pm 0.026$ \\
                           &                          & cnn + img trans & $0.954 \pm 0.016$ & $0.951 \pm 0.014$ & $0.937 \pm 0.009$  & $0.931 \pm 0.017$  & $0.949 \pm 0.009$ \\\midrule
\multirow{6}{*}{500 data}  & \multirow{3}{*}{no crop} & equi            & $0.994 \pm 0.004$ & $0.990 \pm 0.005$ & $0.984 \pm 0.006$  & $0.977 \pm 0.001$  & $0.991 \pm 0.002$ \\
                           &                          & cnn             & $0.760 \pm 0.041$ & $0.760 \pm 0.051$ & $0.771 \pm 0.058$  & $0.772 \pm 0.019$  & $0.745 \pm 0.051$ \\
                           &                          & cnn + img trans & $0.974 \pm 0.006$ & $0.974 \pm 0.011$ & $0.959 \pm 0.013$  & $0.952 \pm 0.010$  & $0.965 \pm 0.012$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.994 \pm 0.003$ & $0.992 \pm 0.003$ & $0.986 \pm 0.004$  & $0.994 \pm 0.003$  & $0.991 \pm 0.005$ \\
                           &                          & cnn             & $0.861 \pm 0.018$ & $0.874 \pm 0.015$ & $0.860 \pm 0.015$  & $0.869 \pm 0.014$  & $0.841 \pm 0.009$ \\
                           &                          & cnn + img trans & $0.987 \pm 0.003$ & $0.989 \pm 0.002$ & $0.991 \pm 0.002$  & $0.972 \pm 0.008$  & $0.982 \pm 0.007$ \\\midrule
\multirow{6}{*}{1000 data} & \multirow{3}{*}{no crop} & equi            & $0.989 \pm 0.005$ & $0.990 \pm 0.003$ & $0.987 \pm 0.011$  & $0.995 \pm 0.002$  & $0.991 \pm 0.004$ \\
                           &                          & cnn             & $0.861 \pm 0.015$ & $0.860 \pm 0.030$ & $0.841 \pm 0.030$  & $0.856 \pm 0.022$  & $0.880 \pm 0.015$ \\
                           &                          & cnn + img trans & $0.990 \pm 0.005$ & $0.992 \pm 0.003$ & $0.975 \pm 0.004$  & $0.991 \pm 0.004$  & $0.991 \pm 0.004$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.996 \pm 0.002$ & $0.998 \pm 0.001$ & $0.990 \pm 0.002$  & $0.990 \pm 0.004$  & $0.998 \pm 0.001$ \\
                           &                          & cnn             & $0.937 \pm 0.018$ & $0.939 \pm 0.020$ & $0.942 \pm 0.019$  & $0.946 \pm 0.012$  & $0.956 \pm 0.017$ \\
                           &                          & cnn + img trans & $0.994 \pm 0.003$ & $0.989 \pm 0.004$ & $0.994 \pm 0.001$  & $0.984 \pm 0.007$  & $0.991 \pm 0.001$ \\\bottomrule
\toprule
\multicolumn{3}{c}{corruption}                                          & two light color   & two specular      & squeeze            & reflect            & condition reverse \\\midrule
\multirow{6}{*}{100 data}  & \multirow{3}{*}{no crop} & equi            & $0.841 \pm 0.023$ & $0.864 \pm 0.020$ & $0.694 \pm 0.015$  & $0.877 \pm 0.017$  & $0.387 \pm 0.034$ \\
                           &                          & cnn             & $0.369 \pm 0.030$ & $0.425 \pm 0.016$ & $0.421 \pm 0.022$  & $0.425 \pm 0.014$  & $0.221 \pm 0.019$ \\
                           &                          & cnn + img trans & $0.584 \pm 0.081$ & $0.631 \pm 0.079$ & $0.595 \pm 0.062$  & $0.645 \pm 0.078$  & $0.381 \pm 0.027$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.885 \pm 0.009$ & $0.906 \pm 0.018$ & $0.757 \pm 0.016$  & $0.916 \pm 0.016$  & $0.405 \pm 0.012$ \\
                           &                          & cnn             & $0.515 \pm 0.060$ & $0.506 \pm 0.062$ & $0.487 \pm 0.053$  & $0.521 \pm 0.067$  & $0.316 \pm 0.035$ \\
                           &                          & cnn + img trans & $0.790 \pm 0.040$ & $0.799 \pm 0.032$ & $0.624 \pm 0.068$  & $0.810 \pm 0.035$  & $0.391 \pm 0.018$ \\\midrule
\multirow{6}{*}{200 data}  & \multirow{3}{*}{no crop} & equi            & $0.937 \pm 0.006$ & $0.944 \pm 0.006$ & $0.865 \pm 0.006$  & $0.937 \pm 0.004$  & $0.447 \pm 0.026$ \\
                           &                          & cnn             & $0.540 \pm 0.032$ & $0.547 \pm 0.037$ & $0.519 \pm 0.029$  & $0.560 \pm 0.036$  & $0.287 \pm 0.023$ \\
                           &                          & cnn + img trans & $0.842 \pm 0.021$ & $0.836 \pm 0.036$ & $0.697 \pm 0.068$  & $0.827 \pm 0.038$  & $0.452 \pm 0.014$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.961 \pm 0.008$ & $0.969 \pm 0.011$ & $0.879 \pm 0.018$  & $0.971 \pm 0.004$  & $0.467 \pm 0.020$ \\
                           &                          & cnn             & $0.710 \pm 0.051$ & $0.720 \pm 0.026$ & $0.664 \pm 0.039$  & $0.686 \pm 0.035$  & $0.412 \pm 0.048$ \\
                           &                          & cnn + img trans & $0.939 \pm 0.017$ & $0.937 \pm 0.018$ & $0.820 \pm 0.038$  & $0.936 \pm 0.020$  & $0.454 \pm 0.025$ \\\midrule
\multirow{6}{*}{500 data}  & \multirow{3}{*}{no crop} & equi            & $0.989 \pm 0.002$ & $0.989 \pm 0.005$ & $0.944 \pm 0.010$  & $0.985 \pm 0.005$  & $0.507 \pm 0.008$ \\
                           &                          & cnn             & $0.714 \pm 0.035$ & $0.750 \pm 0.049$ & $0.715 \pm 0.050$  & $0.752 \pm 0.031$  & $0.504 \pm 0.036$ \\
                           &                          & cnn + img trans & $0.962 \pm 0.010$ & $0.966 \pm 0.008$ & $0.919 \pm 0.010$  & $0.962 \pm 0.013$  & $0.511 \pm 0.013$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.992 \pm 0.004$ & $0.994 \pm 0.003$ & $0.945 \pm 0.020$  & $0.996 \pm 0.001$  & $0.527 \pm 0.020$ \\
                           &                          & cnn             & $0.859 \pm 0.015$ & $0.857 \pm 0.009$ & $0.827 \pm 0.023$  & $0.842 \pm 0.016$  & $0.672 \pm 0.011$ \\
                           &                          & cnn + img trans & $0.987 \pm 0.003$ & $0.977 \pm 0.011$ & $0.952 \pm 0.006$  & $0.982 \pm 0.005$  & $0.524 \pm 0.021$ \\\midrule
\multirow{6}{*}{1000 data} & \multirow{3}{*}{no crop} & equi            & $0.991 \pm 0.001$ & $0.987 \pm 0.005$ & $0.974 \pm 0.007$  & $0.995 \pm 0.002$  & $0.480 \pm 0.017$ \\
                           &                          & cnn             & $0.870 \pm 0.010$ & $0.864 \pm 0.013$ & $0.844 \pm 0.027$  & $0.864 \pm 0.014$  & $0.619 \pm 0.029$ \\
                           &                          & cnn + img trans & $0.990 \pm 0.005$ & $0.990 \pm 0.005$ & $0.961 \pm 0.011$  & $0.977 \pm 0.012$  & $0.487 \pm 0.013$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.996 \pm 0.001$ & $0.999 \pm 0.001$ & $0.971 \pm 0.004$  & $0.995 \pm 0.004$  & $0.494 \pm 0.015$ \\
                           &                          & cnn             & $0.930 \pm 0.013$ & $0.957 \pm 0.018$ & $0.924 \pm 0.012$  & $0.940 \pm 0.014$  & $0.814 \pm 0.010$ \\
                           &                          & cnn + img trans & $0.994 \pm 0.003$ & $0.987 \pm 0.003$ & $0.981 \pm 0.007$  & $0.991 \pm 0.001$  & $0.510 \pm 0.015$ \\\bottomrule\toprule
\multicolumn{3}{c}{corruption}                                          & side              & side, grid        & side, light effect & side, squeeze      & side, reflect     \\\midrule
\multirow{6}{*}{100 data}  & \multirow{3}{*}{no crop} & equi            & $0.515 \pm 0.021$ & $0.501 \pm 0.024$ & $0.497 \pm 0.014$  & $0.549 \pm 0.034$  & $0.526 \pm 0.022$ \\
                           &                          & cnn             & $0.441 \pm 0.022$ & $0.436 \pm 0.028$ & $0.431 \pm 0.021$  & $0.442 \pm 0.021$  & $0.441 \pm 0.013$ \\
                           &                          & cnn + img trans & $0.454 \pm 0.045$ & $0.489 \pm 0.031$ & $0.437 \pm 0.051$  & $0.474 \pm 0.058$  & $0.455 \pm 0.058$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.645 \pm 0.024$ & $0.647 \pm 0.030$ & $0.657 \pm 0.026$  & $0.639 \pm 0.042$  & $0.651 \pm 0.033$ \\
                           &                          & cnn             & $0.491 \pm 0.041$ & $0.486 \pm 0.052$ & $0.494 \pm 0.042$  & $0.457 \pm 0.047$  & $0.496 \pm 0.055$ \\
                           &                          & cnn + img trans & $0.554 \pm 0.031$ & $0.516 \pm 0.065$ & $0.566 \pm 0.036$  & $0.459 \pm 0.046$  & $0.552 \pm 0.065$ \\\midrule
\multirow{6}{*}{200 data}  & \multirow{3}{*}{no crop} & equi            & $0.694 \pm 0.033$ & $0.691 \pm 0.034$ & $0.686 \pm 0.037$  & $0.707 \pm 0.028$  & $0.692 \pm 0.044$ \\
                           &                          & cnn             & $0.556 \pm 0.017$ & $0.555 \pm 0.030$ & $0.572 \pm 0.019$  & $0.551 \pm 0.024$  & $0.571 \pm 0.015$ \\
                           &                          & cnn + img trans & $0.635 \pm 0.046$ & $0.639 \pm 0.019$ & $0.634 \pm 0.037$  & $0.565 \pm 0.064$  & $0.629 \pm 0.041$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.801 \pm 0.028$ & $0.786 \pm 0.022$ & $0.771 \pm 0.021$  & $0.777 \pm 0.019$  & $0.800 \pm 0.006$ \\
                           &                          & cnn             & $0.647 \pm 0.036$ & $0.667 \pm 0.031$ & $0.634 \pm 0.037$  & $0.594 \pm 0.057$  & $0.636 \pm 0.036$ \\
                           &                          & cnn + img trans & $0.737 \pm 0.011$ & $0.770 \pm 0.010$ & $0.732 \pm 0.012$  & $0.739 \pm 0.022$  & $0.779 \pm 0.014$ \\\midrule
\multirow{6}{*}{500 data}  & \multirow{3}{*}{no crop} & equi            & $0.826 \pm 0.031$ & $0.815 \pm 0.019$ & $0.824 \pm 0.032$  & $0.845 \pm 0.018$  & $0.819 \pm 0.033$ \\
                           &                          & cnn             & $0.720 \pm 0.029$ & $0.694 \pm 0.028$ & $0.701 \pm 0.037$  & $0.702 \pm 0.035$  & $0.711 \pm 0.045$ \\
                           &                          & cnn + img trans & $0.851 \pm 0.023$ & $0.825 \pm 0.059$ & $0.797 \pm 0.004$  & $0.766 \pm 0.010$  & $0.850 \pm 0.016$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.911 \pm 0.013$ & $0.906 \pm 0.008$ & $0.912 \pm 0.016$  & $0.896 \pm 0.007$  & $0.905 \pm 0.005$ \\
                           &                          & cnn             & $0.771 \pm 0.019$ & $0.790 \pm 0.025$ & $0.794 \pm 0.022$  & $0.771 \pm 0.020$  & $0.791 \pm 0.017$ \\
                           &                          & cnn + img trans & $0.954 \pm 0.009$ & $0.950 \pm 0.017$ & $0.951 \pm 0.011$  & $0.935 \pm 0.025$  & $0.945 \pm 0.018$ \\\midrule
\multirow{6}{*}{1000 data} & \multirow{3}{*}{no crop} & equi            & $0.919 \pm 0.011$ & $0.924 \pm 0.007$ & $0.914 \pm 0.006$  & $0.922 \pm 0.010$  & $0.920 \pm 0.012$ \\
                           &                          & cnn             & $0.807 \pm 0.031$ & $0.849 \pm 0.019$ & $0.830 \pm 0.011$  & $0.829 \pm 0.019$  & $0.826 \pm 0.030$ \\
                           &                          & cnn + img trans & $0.926 \pm 0.018$ & $0.940 \pm 0.005$ & $0.942 \pm 0.010$  & $0.930 \pm 0.006$  & $0.942 \pm 0.011$ \\\cmidrule(l){2-8}
                           & \multirow{3}{*}{crop}    & equi            & $0.962 \pm 0.008$ & $0.956 \pm 0.005$ & $0.954 \pm 0.014$  & $0.945 \pm 0.010$  & $0.960 \pm 0.006$ \\
                           &                          & cnn             & $0.914 \pm 0.002$ & $0.905 \pm 0.009$ & $0.925 \pm 0.005$  & $0.892 \pm 0.016$  & $0.916 \pm 0.007$ \\
                           &                          & cnn + img trans & $0.985 \pm 0.003$ & $0.986 \pm 0.004$ & $0.972 \pm 0.008$  & $0.979 \pm 0.004$  & $0.985 \pm 0.005$ \\\bottomrule
\end{tabular}
}
\end{table}
